A Little Goes a Long Way: Efficient Long Context Training and Inference with Partial Contexts

Training and serving long-context large language models (LLMs) incurs substantial overhead. To address this, two critical steps are often required: a pretrained LLM typically undergoes a separate stage for context length extension by training on long-context data, followed by architectural modifications to reduce the overhead of KV cache during serving. This paper argues that integrating length extension with a GPU-friendly KV cache reduction architecture not only reduces training overhead during length extension, but also achieves better long-context performance. This leads to our proposed LongGen, which finetunes a pretrained LLM into an efficient architecture during length extension. LongGen builds on three key insights: (1) Sparse attention patterns, such as window attention (attending to recent tokens), attention sink (initial ones), and blockwise sparse attention (strided token blocks) are well-suited for building efficient long-context models, primarily due to their GPU-friendly memory access patterns, enabling efficiency gains not just theoretically but in practice as well. (2) It is essential for the model to have direct access to all tokens. A hybrid architecture with 1/3 full attention layers and 2/3 efficient ones achieves a balanced trade-off between efficiency and long-context performance. (3) Lightweight training on 5B long-context data is sufficient to extend the hybrid model's context length from 4K to 128K. We evaluate LongGen on both Llama-2 7B and Llama-2 70B, demonstrating its effectiveness across different scales. During training with 128K-long contexts, LongGen achieves 1.55x training speedup and reduces wall-clock time by 36%, compared to a full-attention baseline. During inference, LongGen reduces KV cache memory by 62%, achieving 1.67x prefilling speedup and 1.41x decoding speedup.

==> text/old_abstract.tex <==

\hao{comments can be hidden by uncommenting line 22 of macros.tex.
you can add your comments with \suyu
}
\hao{general thoughts on the abstract:
i actually like of flow of the intro better---it is very clear that we sit in the middle of length extension (which involves heavy training/finetuning and does not address the memory issue) and kv cache compression (which usually hurts the performance).
my main concern is that we should tone down \name as a new transformer architecture variant, since the key component of \name, window and sink, are both established. we should not worry about a lack of "novelty" either, since it is really elegant to make a simple and robust architecture achieve both long context and kv chace compression, w/o the hacky tricks.
}
We introduce an efficient transformer architecture, \name \hao{why this acronym?}, for better large language model (LLM) training and inference on long context \hao{can we be more specific? our highlight is a hybrid architecture that can achieve length extension and kv cache reduction at the same time}.
It inherits standard transformer architecture but enforces sparsity in certain layers by retaining only partial contexts from specific positions.
Starting from any existing pretrained model, \name can learn to condense information of the entire sequence with partial contexts.
\hao{re the prev couple of sents---we should be more concrete, since our method can be clearly described in one/two sentences, which i woud do}
It does not require pretraining from scratch and instead, only demands a light-weight continuous training on 3B tokens \hao{\% amount of the pretraining data, XX GPU hours} to extend the context length from 4k to 128k. 
During inference, \name enjoys the merits of sparse training and effortlessly \hao{<- i'd be more concrete---\name uses full contexts}reduces memory consumption with only XX\% KV cache stored.
We conduct experiments to extend the context length of a 7B and 70B llama model by training them on 128k context length.
To explore how different sparsity levels affect long context capability, we alternate the number of layers with partial contexts and set the remaining as full context layers.
Evaluation are done on multiple long-context benchmarks, which indicates that \name could achieve comparable performances with standard transformers even with 2/3 of its layers being with partial context.
Specifically, it achieves a XX times speedup on inference throughput without hurting short-context and long-context capabilities.
Our analysis also suggests that needle retrieval is spoiled, shedding light on why evaluation on other benchmarks is extremely necessary. 

